Optimal Dynamic Regret in Exp-Concave Online Learning

We consider the problem of the Zinkevich (2003)-style dynamic regret minimization in online learning with exp-concave losses. We show that whenever improper learning is allowed, a Strongly Adaptive online learner achieves the dynamic regret of $\tilde O^*(n^{1/3}C_n^{2/3} \vee 1)$ where $C_n$ is the total variation (a.k.a. path length) of the an arbitrary sequence of comparators that may not be known to the learner ahead of time. Achieving this rate was highly nontrivial even for squared losses in 1D where the best known upper bound was $O(\sqrt{nC_n} \vee \log n)$ (Yuan and Lamperski, 2019). Our new proof techniques make elegant use of the intricate structures of the primal and dual variables imposed by the KKT conditions and could be of independent interest. Finally, we apply our results to the classical statistical problem of locally adaptive non-parametric regression (Mammen, 1991; Donoho and Johnstone, 1998) and obtain a stronger and more flexible algorithm that do not require any statistical assumptions or any hyperparameter tuning.

==> backup.tex <==
\begin{comment}
\section{Performance guarantees for strongly convex losses}
We begin by listing all the assumptions we make about the loss functions.

\begin{enumerate}
    \item [SC-1] The loss functions $f_t(\bs x) : \mathbb{R}^d \rightarrow \mathbb R$ are $H$-strongly convex across the entire $\mathbb{R}^d$.
    
    \item [SC-2] The loss functions $f_t(\bs x) : \mathbb{R}^d \rightarrow \mathbb R$ are $\beta$-strongly smooth across the entire $\mathbb{R}^d$.
    
    \item [SC-3] The outputs of learner belongs to a convex decision set $\mathcal D \subset \mathbb{R}^d$. Further the gradient of loss functions satisfy $\|\grad f_t(\bs x)\|_2 \le G$ for all $\bs x \in \mathcal D$. 
\end{enumerate}


For the sake of simplicity, we first present the results in one dimensional setting and extend it later to higher dimensions.

\subsection{One dimensional setting}
\begin{theorem} \label{thm:sc-1d} ($d=1$) 
By using the base learner as OGD with step sizes $\zeta_t = 1/Ht$, decision set $\cD$ and choosing learning rate $\eta = H/G^2$, \ALG{} guarantees $R_n(C_n) = \tilde O \left( n^{1/3}C_n^{2/3} \right)$.
\end{theorem}

We need some technical lemmas to prove the above result. We start by inspecting the KKT conditions of the offline optimal solution.
\begin{lemma} \label{lem:kkt-sc} (\textbf{characterization of offline optimal}) 
Let $u_1,\ldots,u_n$ be the optimal solutions of:
\begin{equation}
\begin{aligned}
\min_{\tilde u_1,\ldots,\tilde u_n} \quad & \sum_{t=1}^{n} f_t(\tilde u_t)\\
\textrm{s.t.} \quad & \sum_{t=2}^{n} |\tilde u_t - \tilde u_{t-1}| \le C_n\\
\end{aligned}
\end{equation}
Then the gradients of the loss functions satisfy $\nabla f_t(u_t) = \lambda \left ( s(u_{t+1} - u_t) - s(u_t - u_{t-1}) \right)$ for all $t \in [n]$ for some $\lambda > 0$ and we take $s(u_1-u_0)$ and $s(u_{n+1} - u_n)$ to be zero.
\end{lemma}
\begin{proof}
Define $\bs z = [u_2-u_1,\ldots,u_n-u_{n-1}]^T$ and $\tilde {\bs z}$ similarly. We can form the Lagrangian as:
\begin{align}
    \mathcal{L}(\tilde{\bs u} , \tilde{\bs z}, \tilde{\bs v}, \tilde{\lambda})
    &= \sum_{t=1}^{n} f_t(\tilde u_t) + \tilde \lambda \left( \sum_{t=1}^{n-1} |\tilde z_t| - C_n\right) + \sum_{t=1}^{n-1} \tilde v_t( \tilde u_{t+1} - \tilde u_t - \tilde z_t),
\end{align}
for dual variables $\tilde \lambda > 0$ and $\tilde {\bs v}$ unconstrained. Let the $(\bs u, \bs z, \bs v, \lambda)$ be the optimal primal and dual variables. By stationarity conditions, we have 
\begin{align}
    \grad f_t(u_t) = v_t - v_{t-1},
\end{align}
where we take $v_0 = v_n = 0$ and
\begin{align}
    v_t = \lambda s(u_{t+1} - u_t).
\end{align}
Combining the above two equations yields the lemma.
\end{proof}

Next we display a regret decomposition which serves a central role in our analysis.
\begin{proposition} \label{prop:regret-decomp} (\textbf{key regret decomposition})
Let $u_1,\ldots,u_n$ be as defined in Lemma \ref{lem:kkt-sc}. Partition the entire horizon $[n]$ into $M$ bins. Let $[i_s, i_t]$ denote the $i^{th}$ bin and let $n_i$ be its length. We only consider partitions that satisfy $|s(u_{i_s} - u_{i_s-1})| = 1$ for all $i_s \neq 1$. Define $\bar u_i = \frac{1}{n_i} \sum_{j=i_s}^{i_t} u_j$ and $\dot u_i = \bar u_i - \frac{1}{n_i \beta} \sum_{j=i_s}^{i_t} \grad f_j(u_j)$ where $\beta$ is as in Assumption SC-2. Let $\hat u_j$ be the prediction made by \ALG{} at time $j$. Then we have,
\begin{align}
    R_n(C_n)
    &\le \sum_{i=1}^{M} \underbrace{\sum_{j=i_s}^{i_t} f_j(\hat u_j) - f_j(\dot u_i)}_{T_{1,i}} + \sum_{i=1}^{M} \underbrace{\sum_{j=i_s}^{i_t} f_j(\dot u_i) - f_j(\bar u_i)}_{T_{2,i}} + \sum_{i=1}^{M} \underbrace{\sum_{j=i_s}^{i_t} f_j(\bar u_i) - f_j(u_j)}_{T_{3,i}}.
\end{align}
\end{proposition}

Now we proceed to bound each of the terms displayed above. 
\begin{lemma} \label{lem:t1-sc} (\textbf{bounding } $T_{1,i}$)
Assume that we run \ALG{} with the settings desrcibed in Theorem \ref{thm:sc-1d}. For any bin $i$ we have,
\begin{align}
    \sum_{j=i_s}^{i_t} f_j(\hat u_j) - f_j(\dot u_i) = O \left(\frac{G^2}{H} \log n \right)
\end{align}
\end{lemma}
\begin{proof}
By Assumption SC-1 and SC-3, the losses $f_j$ are $H/G^2$ exp-concave in the set $\mathcal{D}$. Since all the base OGD subroutines outputs predictions in the set $\mathcal{D}$, from Theorem 3.2 of \citep{hazan2007adaptive} we have
\begin{align}
    \sum_{j=i_s}^{i_t} f_j(\hat u_j) - f_j(\dot u_i)
    &\le \text{static regret of OGD} + O\left(\frac{G^2}{H} \log n \right).
\end{align}

It follows from Theorem 1 of \citep{hazan2007logregret} that $\text{static regret of OGD } = O\left(\frac{G^2}{H} \log n \right)$.
\end{proof}

\begin{lemma} \label{lem:t2-sc} (\textbf{bounding } $T_{2,i}$)
Define $C_i := \sum_{j=i_s+1}^{i_t} |u_j - u_{j-1}|$, the TV within bin $i$ incurred by the offline optimal solution. Let $\Delta s_i := s(u_{i_t+1} - u_{i_t}) - s(u_{i_s} - u_{i_s - 1})$. We have
\begin{align}
    \sum_{j=i_s}^{i_t} f_j(\dot u_i) - f_j(\bar u_i)
    &\le \frac{-\lambda^2 (\Delta s_i)^2}{2n_i \beta} + \lambda |\Delta s_i| C_i.
\end{align}
\end{lemma}
\begin{proof}
Let $g(x)$ be a $\alpha$-strongly smooth function. Let $x^+ = x - \mu \grad f(x)$ for some $\mu > 0$. Then we have
\begin{align}
    g(x^+) - g(x)
    &\le (\grad g(x))^2 \left(\frac{\alpha}{2} \mu^2  - \mu \right),\\
    &= \frac{-(\grad g(x))^2}{2\alpha},
\end{align}
by choosing $\mu = 1/\alpha$. By taking $g(x) = \sum_{j=i_s}^{i_t} f_j(x)$ and noting that $g$ is $n_i \beta$ gradient Lipschitz due to Assumption SC-2, we get
\begin{align}
    T_{2,i}
    &:=\sum_{j=i_s}^{i_t} f_j(\dot u_i) - f_j(\bar u_i),\\
    &\le \frac{-\left(\sum_{j=i_s}^{i_t} \grad f_j(\bar u_i) \right)^2}{2 n_i \beta},\\
    &= \frac{-1}{2n_i \beta} \left(\sum_{j=i_s}^{i_t} \grad f_j( u_j) + \grad f_j(\bar u_i) - \grad f_j( u_j)\right)^2,\\
    &\le \frac{-1}{2n_i \beta} \left(\sum_{j=i_s}^{i_t} \grad f_j(u_j) \right)^2 + \frac{1}{n_i \beta} \left|\sum_{j=i_s}^{i_t} \grad f_j(u_j) \right| \left| \sum_{j=i_s}^{i_t} \grad f_j(\bar u_i) - \grad f_j(u_j) \right|.
\end{align}
From the KKT conditions in Lemma \ref{lem:kkt-sc} we have $\sum_{j=i_s}^{i_t} \grad f_j(u_j) = \lambda \Delta s_i$. Since $f_j$ are $\beta$-gradient Lipschitz and $|\bar u_i - u_j | \le C_i$, we also have 
\begin{align}
  \left| \sum_{j=i_s}^{i_t} \grad f_j(\bar u_i) - \grad f_j(u_j) \right| &\le  n_i \beta C_i  
\end{align}
Substituting these we get,
\begin{align}
    T_{2,i}
    &\le \frac{-\lambda^2 (\Delta s_i)^2}{2n_i \beta} + \lambda |\Delta s_i| C_i.
\end{align}
\end{proof}

\begin{lemma} \label{lem:t3-sc} (\textbf{bounding }$T_{3,i}$) Let $C_i$ and $\Delta s_i$ be as in Lemma \ref{lem:t2-sc}.\\
\textbf{case(a)} If $|\Delta s_i| > 0$ then we have,
\begin{align}
    \sum_{j=i_s}^{i_t} f_j(\bar u_i) - f_j(u_j)
    &\le  \frac{\beta n_i C_i^2}{2} + 3\lambda C_i.
\end{align}
\textbf{case(b)} If $\Delta s_i = 0$ with $s(u_{i_s} - u_{i_s-1}) = s(u_{i_s} - u_{i_s-1}) = 1$ and the offline optimal $\bs u$ is non-decreasing within bin $i$, then
\begin{align}
    \sum_{j=i_s}^{i_t} f_j(\bar u_i) - f_j(u_j)
    &\le  \frac{\beta n_i C_i^2}{2}.
\end{align}
\textbf{case(c)} If $\Delta s_i = 0$ with $s(u_{i_s} - u_{i_s-1}) = s(u_{i_s} - u_{i_s-1}) = -1$ and the offline optimal $\bs u$ is non-increasing within bin $i$, then
\begin{align}
    \sum_{j=i_s}^{i_t} f_j(\bar u_i) - f_j(u_j)
    &\le  \frac{\beta n_i C_i^2}{2}.
\end{align}

\end{lemma}
\begin{proof}
Due to strong smoothness, we have
\begin{align}
    T_{3,i}
    &:=\sum_{j=i_s}^{i_t} f_j(\bar u_i) - f_j(u_j),\\
    &\le \sum_{j=i_s}^{i_t} \grad f_j(u_j) (\bar u_i - u_j) + \frac{\beta}{2} (\bar u_i - u_j)^2,\\
    &\le \frac{\beta n_i C_i^2}{2} + \sum_{j=i_s}^{i_t} \grad f_j(u_j) (\bar u_i - u_j).
\end{align}
Now by expanding the second term and using the structure of gradients as in Lemma \ref{lem:kkt-sc} followed by a regrouping of the terms in the summation we can write,
\begin{align}
    \sum_{j=i_s}^{i_t} \grad f_j(u_j) (\bar u_i - u_j)
    &= \lambda \left( s(u_{i_s} - u_{i_s-1}) (u_{i_s} - \bar u_i) - s(u_{i_t + 1} - u_{i_t}) (u_{i_t} - \bar u_i)\right) + \lambda \sum_{j=i_s+1}^{i_t} |u_j - u_{j-1}|,\\
    &\le \lambda \left( s(u_{i_s} - u_{i_s-1}) (u_{i_s} - \bar u_i) - s(u_{i_t + 1} - u_{i_t}) (u_{i_t} - \bar u_i)\right) + \lambda C_i. \label{eqn:inter}
\end{align}

Now we consider three cases. 

\textbf{case(a) }When $|\Delta s_i| > 0$, then by triangle inequality we have \\$\lambda \left( s(u_{i_s} - u_{i_s-1}) (u_{i_s} - \bar u_i) - s(u_{i_t + 1} - u_{i_t}) (u_{i_t} - \bar u_i)\right) \le 2\lambda C_i$.

\textbf{case(b) and case (c) }In both these cases, we have $\lambda \left( s(u_{i_s} - u_{i_s-1}) (u_{i_s} - \bar u_i) - s(u_{i_t + 1} - u_{i_t}) (u_{i_t} - \bar u_i)\right) = -\lambda C_i$ which cancels with the additive term in Eq. \eqref{eqn:inter} . Putting everything together now yields the lemma.

\end{proof}

Next, we describe a partition of the optimal solution sequence which is similar to that used in \citep{arrows2019}. We also provide the proof for completeness.
\begin{lemma}(\textbf{key partition}) \label{cor:part-1d}
Initialize $\cP \leftarrow \Phi$. Starting from time 1, spawn a new bin $[i_s,i_t]$ whenever $\sum_{j=i_s+1}^{i_t+1} | u_j -  u_{j-1} | > B/\sqrt{n_i}$, where $n_i = i_t - i_s + 1$. Add the spawned bin $[i_s,i_t]$ to $\cP$.

Let $M:=|\cP|$. We have $M = O(n^{1/3}C_n^{2/3})$.
\end{lemma}
\begin{proof}
Let's use the notation $TV[a,b]$ to denote the TV incurred by the optimal solution sequence in the interval $[a,b]$. Let $\cP = \{[\ubar t_1, \bar t_1],\ldots,[\ubar t_M, \bar t_M] \}$ with $\ubar t_1 := 1$ and $\bar t_M := n$. Let $n_j:= \bar t_j - \ubar t_j + 1$ We have,

\begin{align}
    \sum_{j=1}^{M-1} TV[\ubar t_j, \bar t_j+1] \le C_n.
\end{align}

By construction we have $TV[\ubar t_j, \bar t_j+1] > B/\sqrt{n_j}$. So,

\begin{align}
    C_n
    &\ge \sum_{j=1}^{M-1} B/\sqrt{n_j},\\
    &\ge (M-1)^{3/2}B/\sqrt{n},
\end{align}
where the last line follows by Jensen's inequality. Rearranging gives the bound on $M$.
\end{proof}

\begin{proof}\textbf{of Theorem} \ref{thm:sc-1d}. We start from the regret decomposition in Proposition \ref{prop:regret-decomp}. First we handle the case(a) in Lemma \ref{lem:t3-sc} where $|\Delta s_i| > 0$.  Define $T_i:= \sum_{j=i_s}^{i_t} f_j(\hat u_j) - f_j(u_j)$. From Lemmas \ref{lem:t1-sc}, \ref{lem:t2-sc} and \ref{lem:t3-sc} we have
\begin{align}
    T_i
    &\le  O\left(\frac{G^2}{H} \log n \right) - \frac{\lambda^2 (\Delta s_i)^2}{2n_i \beta} + \lambda |\Delta s_i| C_i + \frac{\beta n_i C_i^2}{2} + 3\lambda C_i,\\
    &\le_{(a)}  O\left(\frac{G^2}{H} \log n \right) + \frac{\beta n_i C_i^2}{2} + 5 \lambda C_i  - \frac{\lambda^2 (\Delta s_i)^2}{2n_i \beta},\\
    &= O\left(\frac{G^2}{H} \log n \right) + \frac{\beta n_i C_i^2}{2} + \frac{25 \beta n_i C_i^2}{2(\Delta s_i)^2} - \left(\frac{\lambda \Delta s_i}{\sqrt{2 n_i \beta}} - \frac{5C_i \sqrt{n_i \beta}}{\Delta s_i \sqrt 2} \right)^2,\\
    &\le_{(b)} O\left(\frac{G^2}{H} \log n \right) + 26 \beta n_i C_i^2,
\end{align}
where  in line (a) we used the fact that $|\Delta s_i| \le 2$. In line (b) we used the fact that $|\Delta s_i| \ge 1$ if $|\Delta s_i| \neq 0$. (Recall properties of the partition in Proposition \ref{prop:regret-decomp}). 

To handle case(b) and case (c) in Lemma \ref{lem:t3-sc} where $\Delta s_i = 0$ and monotonic, it is immediate that $T_i \le  O\left(\frac{G^2}{H} \log n \right) + \frac{\beta n_i C_i^2}{2}$.

Consider the case when $\Delta s_i = 0$ with $s(u_{i_s} - u_{i_s-1}) = s(u_{i_t+1} - u_{i_t}) = -1$ and the offline optimal $\bs u$ is non-decreasing within bin $i$. If the sequence is constant within the bin, then trivially we have $T_i = O\left(\frac{G^2}{H} \log n \right)$ due to Strongly Adaptive regret. Otherwise, we the split the original bin into two sub-bins $[i_s,k]$ and $[k+1,i_t]$ such that $s(u_{k+1} - u_k) = 1$. Then the two sub-bins falls into the category of case (a) in Lemma \ref{lem:t3-sc}. By bounding the regret within each sub-bin separately by following the previous arguments and adding them up, we can get $T_i \le  O\left(\frac{G^2}{H} \log n \right) + \frac{\beta n_i C_i^2}{2}$. for the original bin. The arguments for the case when $\Delta s_i = 0$ with $s(u_{i_s} - u_{i_s-1}) = s(u_{i_t+1} - u_{i_t}) = 1$ and the offline optimal $\bs u$ is non-increasing within bin $i$ are similar.

To handle the case when  $\Delta s_i = 0$ and the optimal sequence is \emph{not} monotonic, we split the bin into two parts. Consider the case $s(u_{i_t + 1} - u_{i_t}) = s(u_{i_s} - u_{i_s-1}) = 1$. We can split $\bs u_{i_s:i_t}$ as $\bs u_{i_s:k}$ and $\bs u_{k+1:i_t}$ such that the sequence $\bs u_{i_s:k}$ is non-decreasing and $s(u_{k+1} - u_k) = -1$. Notice that both the sub-bins  $\bs u_{i_s:k}$ and $\bs u_{k+1:i_t}$ now falls into the category of case(a). Adding the bounds within these sub-bins by following the treatment above yields $T_i \le O\left(\frac{G^2}{H} \log n \right) + 26 \beta n_i C_i^2$. The arguments for the scenario $s(u_{i_t + 1} - u_{i_t}) = s(u_{i_s} - u_{i_s-1}) = -1$ are similar.

Now using the partitioning scheme described in Corollary \ref{cor:part-1d}, where we have the TV within each bin $C_i \le \frac{B}{\sqrt{n_i}}$, and number of bins $M = O \left(n^{1/3}C_n^{2/3}\right)$, we see that
\begin{align}
    R_n(C_n)
    &\le \sum_{i=1}^{M} O\left(\frac{G^2}{H} \log n \right) + 26 \beta n_i C_i^2,\\
    &= \tilde O \left( \left(\frac{G^2}{H} + \beta \right) n^{1/3}C_n^{2/3} \right).
\end{align}

\end{proof}
\end{comment}


\begin{comment}
\section{Multi-dimensional setting: Strongly Convex losses}
\begin{theorem}\label{thm:sc-d}
By using the base learner as OGD with step sizes $\eta_t = 1/Ht$ with decision set $\cD$ and  choosing learning rate $\eta = H/G^2$, \ALG{} guarantees $R_n(C_n) = \tilde O \left(d n^{1/3}C_n^{2/3} \right)$.
\end{theorem}

\begin{lemma} \label{lem:kkt-sc-d} (\textbf{characterization of offline optimal}) 
Let $\bs u_1,\ldots, \bs u_n$ be the optimal solutions of:
\begin{equation}
\begin{aligned}
\min_{\tilde {\bs u}_1,\ldots,\tilde {\bs u}_n} \quad & \sum_{t=1}^{n} f_t(\tilde {\bs u}_t)\\
\textrm{s.t.} \quad & \sum_{t=2}^{n} \|\tilde {\bs u}_t - \tilde {\bs u}_{t-1}\|_1 \le C_n\\
\end{aligned}
\end{equation}
Then the gradients of the loss functions satisfy $\nabla f_t({\bs u}_t) = \lambda \left ( s({\bs u}_{t+1} - {\bs u}_t) - s({\bs u}_t - {\bs u}_{t-1}) \right)$ for all $t \in [n]$ for some $\lambda > 0$ and we take $s({\bs u}_1-{\bs u}_0)$ and $s({\bs u}_{n+1} - {\bs u}_n)$ to be zero.
\end{lemma}
Proof of the above lemma is similar to that of Lemma \ref{lem:kkt-sc} and hence skipped.

\begin{proposition} \label{prop:regret-decomp-d} (\textbf{key regret decomposition})
Let $\bs u_1,\ldots,\bs u_n$ be as defined in Lemma \ref{lem:kkt-sc-d}. Partition the entire horizon $[n]$ into $M$ bins. Let $[i_s, i_t]$ denote the $i^{th}$ bin and let $n_i$ be its length. Define $\bar {\bs u}_i = \frac{1}{n_i} \sum_{j=i_s}^{i_t} \bs u_j$ and $\dot {\bs u}_i = \bar { \bs u}_i - \frac{1}{n_i \beta} \sum_{j=i_s}^{i_t} \grad f_j(\bs u_j)$ where $\beta$ is as in Assumption SC-2. Let $\hat {\bs u}_j$ be the prediction made by \ALG{} at time $j$. Then we have,
\begin{align}
    R_n(C_n)
    &\le \sum_{i=1}^{M} \underbrace{\sum_{j=i_s}^{i_t} f_j(\hat {\bs u}_j) - f_j(\dot {\bs u}_i)}_{T_{1,i}} + \sum_{i=1}^{M} \underbrace{\sum_{j=i_s}^{i_t} f_j(\dot {\bs u}_i) - f_j(\bar {\bs u}_i)}_{T_{2,i}} + \sum_{i=1}^{M} \underbrace{\sum_{j=i_s}^{i_t} f_j(\bar {\bs u}_i) - f_j({\bs u}_j)}_{T_{3,i}}.
\end{align}
\end{proposition}

\begin{lemma} \label{lem:t1-sc-d} (\textbf{bounding } $T_{1,i}$)
For any bin $i$ we have,
\begin{align}
    \sum_{j=i_s}^{i_t} f_j(\hat {\bs u}_j) - f_j(\dot {\bs u}_i) = O \left(\frac{G^2}{H} \log n \right)
\end{align}
\end{lemma}
The above result follows directly from SA regret bounds as in the proof of Lemma \ref{lem:t1-sc}.

\begin{lemma} \label{lem:t2-sc-d} (\textbf{bounding } $T_{2,i}$)
Define  $C_i = \sum_{j=i_s+1}^{i_t} \|\bs u_{j} - \bs u_{j-1} \|_1$, the TV within bin $i$ incurred by the offline optimal solution. Let $\Delta \bs s_i := \bs s(u_{i_t+1} - u_{i_t}) - \bs s(u_{i_s} - u_{i_s - 1})$. We have
\begin{align}
    \sum_{j=i_s}^{i_t} f_j(\dot {\bs u}_i) - f_j(\bar {\bs u}_i)
    &\le \frac{-\lambda^2 \|\Delta \bs s_i\|_2^2}{2n_i \beta} + \lambda \|\Delta \bs s_i\|_2 C_i.
\end{align}
\end{lemma}
\begin{proof}
Let $g(\bs x)$ be a $\alpha$-strongly smooth function. Let $\bs x^+ = \bs x - \mu \grad f(\bs x)$ for some $\mu > 0$. Then we have
\begin{align}
    g(\bs x^+) - g(\bs x)
    &\le \|\grad g(\bs x)\|_2^2 \left(\frac{\alpha}{2} \mu^2  - \mu \right),\\
    &= \frac{-\|\grad g(\bs x)\|_2^2}{2\alpha},
\end{align}
by choosing $\mu = 1/\alpha$. By taking $g(x) = \sum_{j=i_s}^{i_t} f_j(\bs x)$ and noting that $g$ is $n_i \beta$ gradient Lipschitz due to Assumption SC-2, we get
\begin{align}
    T_{2,i}
    &:=\sum_{j=i_s}^{i_t} f_j(\dot {\bs u}_i) - f_j(\bar {\bs u}_i),\\
    &\le \frac{-\left\|\sum_{j=i_s}^{i_t} \grad f_j(\bar {\bs u}_i) \right\|_2^2}{2 n_i \beta},\\
    &= \frac{-1}{2n_i \beta} \left\|\sum_{j=i_s}^{i_t} \grad f_j( {\bs u}_j) + \grad f_j(\bar {\bs u}_i) - \grad f_j( {\bs u}_j)\right\|_2^2,\\
    &\le \frac{-1}{2n_i \beta} \left\|\sum_{j=i_s}^{i_t} \grad f_j({\bs u}_j) \right\|_2^2 + \frac{1}{n_i \beta} \left \|\sum_{j=i_s}^{i_t} \grad f_j({\bs u}_j) \right\|_2 \left\| \sum_{j=i_s}^{i_t} \grad f_j(\bar {\bs u}_i) - \grad f_j({\bs u}_j) \right\|_2, \label{eqn:t2-last}
\end{align}
where we used $\langle \bs x, \bs y \rangle \le \|\bs x\|_1 \| \bs y \|_2$. From the KKT conditions in Lemma \ref{lem:kkt-sc} we have $\sum_{j=i_s}^{i_t} \grad f_j({\bs u}_j) = \lambda \Delta \bs s_i$. Since $f_j$ are $\beta$-gradient Lipschitz and $\|\bar {\bs u}_i - {\bs u}_j \|_2 \le \|\bar {\bs u}_i - {\bs u}_j \|_1 \le C_i$, we also have 
\begin{align}
  \left\| \sum_{j=i_s}^{i_t} \grad f_j(\bar {\bs u}_i) - \grad f_j({\bs u}_j) \right\|_2 &\le  n_i \beta C_i.
\end{align}
Substituting these we get,
\begin{align}
    T_{2,i}
    &\le \frac{-\lambda^2 \|\Delta \bs s_i\|_2^2}{2n_i \beta} + \lambda \|\Delta \bs s_i\|_2 C_i.
\end{align}
\end{proof}

\begin{lemma} \label{lem:t3-sc-d} (\textbf{bounding }$T_{3,i}$) Let $C_i$ be as in Lemma \ref{lem:t2-sc-d}. We have,
\begin{align}
    \sum_{j=i_s}^{i_t} f_j(\bar {\bs u}_i) - f_j({\bs u}_j)
    &\le  \frac{\beta n_i C_i^2}{2} + \sum_{j=i_s}^{i_t} \langle \grad f_j({\bs u}_j), \bar {\bs u}_i - {\bs u}_j \rangle.
\end{align}
\end{lemma}
\begin{proof}
Due to strong smoothness, we have
\begin{align}
    T_{3,i}
    &:=\sum_{j=i_s}^{i_t} f_j(\bar {\bs u}_i) - f_j({\bs u}_j),\\
    &\le_{(a)} \sum_{j=i_s}^{i_t} \langle \grad f_j({\bs u}_j), \bar {\bs u}_i - {\bs u}_j \rangle + \frac{\beta}{2} \|\bar {\bs u}_i - {\bs u}_j\|_1^2,\\
    &\le \frac{\beta n_i C_i^2}{2} + \sum_{j=i_s}^{i_t} \langle \grad f_j({\bs u}_j), \bar {\bs u}_i - {\bs u}_j \rangle,
\end{align}
where in line (a) we used $\|\bar {\bs u}_i - {\bs u}_j\|_2 \le \|\bar {\bs u}_i - {\bs u}_j\|_1$.
\end{proof}

Next, describe the partition we will consider. 

\begin{proposition} \label{prop:key-part} (\textbf{key partition})
We form a partition $\cP$ by sequentially executing the following steps.
\begin{enumerate}
    \item[Step 1] Initialize $\cP \leftarrow \Phi$. Starting from time 1, spawn a new bin $[i_s,i_t]$ whenever $\sum_{j=i_s+1}^{i_t+1} \|\bs u_j - \bs u_{j-1} \|_1 > B/\sqrt{n_i}$, where $n_i = i_t - i_s + 1$. Add the spawned bin $[i_s,i_t]$ to $\cP$.
    \item[Step 2] Initialize $\mathcal G \leftarrow \Phi$. Let $\cS$ be the collection of all bins $[i_s,i_t]$ such that $|\Delta \bs s_i[k]| \in [0,1)$ for all coordinates $k \in [d]$ and there exists a coordinate $k'$ such that $|s(\bs u_{i_s}[k'] - \bs u_{i_s-1}[k']) - s(\bs u_{i_r+1}[k'] - \bs u_{i_r}[k'])| \ge 1/2$ and $|s(\bs u_{i_{t}+1}[k'] - \bs u_{i_t}[k']) - s(\bs u_{i_r+1}[k'] - \bs u_{i_r}[k'])| \ge 1/2$ for some $i_r \in (i_s,i_t)$. Split the bin $[i_s,i_t]$ in $\cS$ into two bins $[i_s,i_r]$ and $[i_r+1,i_t]$ and add them $\mathcal G$, where $i_r$ is as described before. If multiple coordinates satisfy the condition, then $i_r$ can be chosen by considering lowest such $k'$. Update $\cP \leftarrow \cP \setminus \cS \cup \mathcal G$.
    \item[Step 3] Let $\mathcal Q \subset \cP \setminus \mathcal G$ be the collection of remaining bins of the form $[i_s,i_t]$ with $|\Delta \bs s_i[k]| \in [0,1)$ for all coordinates $k \in [d]$. Initialize the list $\cT \leftarrow \Phi$. For each $[i_s,i_t] \in \mathcal Q$:
    \begin{enumerate}
        \item Add $i_s,i_t$ to $\cT$ and sort $\cT$ in increasing order.
        \item For $k$ in $1$ to $d$:
    \begin{enumerate}
        \item Let $t_1$ be the smallest time with $i_s \le t_1 < i_t$ such that $\bs u_{t_1}[k] > \bs u_{t_1-1}[k]$. Let $t_2$ be the largest time with $i_s < t_2 \le i_t$ such that $\bs u_{t_2+1}[k] > \bs u_{t_2}[k]$. If $t_1-1 \ge i_s$ add $t_1 - 1$ to $\cT$. If $t_1 < t_2$ add $t_1,t_2$ to $\cT$. If $t_2+1 \le i_t$, add $t_2+1$ to $\cT$. If a time point is added to $\cT$ in this step, we remove $[i_s,i_t]$ from $\cP$.
        
        \item If a time point was added to $\cT$ in previous step, we skip the current step. Otherwise, let $t_1$ be the smallest time with $i_s \le t_1 < i_t$ such that $\bs u_{t_1}[k] < \bs u_{t_1-1}[k]$. Let $t_2$ be the largest time with $i_s < t_2 \le i_t$ such that $\bs u_{t_2+1}[k] < \bs u_{t_2}[k]$. If $t_1-1 \ge i_s$ add $t_1 - 1$ to $\cT$. If $t_1 < t_2$ add $t_1,t_2$ to $\cT$. If $t_2+1 \le i_t$, add $t_2+1$ to $\cT$. If a time point is added to $\cT$ in this step, we remove $[i_s,i_t]$ from $\cP$.
        
        %If $t_1 -1 \ge i_s$ add $(i_s,t_1-1)$ to $\cT$. If $t_1 \le t_2$ add $(t_1,t_2)$ to $\cT$. If $t_2+1 \le i_t$ add $(t_2+1,i_t)$ to $\cT$. If a valid pair is added to $\cT$ in this step, we remove $[i_s,i_t]$ from $\cP$.
    \end{enumerate}
    \end{enumerate}
    
    \item[Step 4] For each entry $t$ in $\cT$:
    \begin{enumerate}
        \item If $t$ appears more than 2 times, delete some occurences of $t$ such that $t$ only appears 2 times in $\cT$. 
    \end{enumerate}
    \item[Step 5] Sort $\cT$ in non-decreasing order. For each consecutive points $s,t \in \mathcal T$, add $[s,t]$ to $\cP$.
\end{enumerate}
\end{proposition}

\begin{lemma} \label{lem:num-bins}
Number of bins in the partition $\cP$ of Proposition \ref{prop:key-part} is at-most $O(d n^{1/3}C_n^{2/3})$.
\end{lemma}
\begin{proof}
Following similar arguments as in the proof of Corollary \ref{cor:part-1d}, it can be shown that the number of bins formed by Step 1 in Proposition \ref{prop:key-part} is $O(n^{1/3}C_n^{2/3})$. Step 2 can only increase the bin count by at-most a factor of 2. In step 3 and step 4, each coordinate can contribute to an increase of $O(n^{1/3}C_n^{2/3})$. Adding the contribution from all coordinates yields the Lemma.
\end{proof}

\begin{proof}\textbf{of Theorem} \ref{thm:sc-d}.
We inherit all the notations of Proposition \ref{prop:key-part}. In the proof we bound the regret incurred within each bin in the partition of Proposition \ref{prop:key-part} and add them up to get the final regret bound. First we consider bins in the partition $\cP$ of the form $[i_s,i_t]$ with $\|\Delta \bs s_i\|_\infty \ge 1/2$. Let the number of such bins be $M_1$. To gain some perspective, notice that all the bins present in $\mathcal G$ at the end of step 2 in Proposition \ref{prop:key-part} satisfies this criteria. There may be other bins that are formed in Step 1 that can also satisfy this condition.

To bound $T_{3,i}$ in Lemma \ref{lem:t3-sc-d}, we inspect the following term and proceed similar to proof of Lemma \ref{lem:t3-sc}.
\begin{align}
    \sum_{j=i_s}^{i_t} \langle \grad f_j({\bs u}_j), \bar {\bs u}_i - {\bs u}_j \rangle
    &=\lambda \left( \langle s( {\bs u}_{i_s} - {\bs u}_{i_s-1}), {\bs u}_{i_s} - \bar {\bs u}_i \rangle - \langle s({\bs u}_{i_t + 1} - {\bs u}_{i_t}) , {\bs u}_{i_t} - \bar {\bs u}_i \rangle \right) \\ &\qquad +\lambda \sum_{j=i_s+1}^{i_t} |{\bs u}_j - {\bs u}_{j-1}|,\\
    &\le \lambda \| s( {\bs u}_{i_s} - {\bs u}_{i_s-1}) \|_\infty \|{\bs u}_{i_s} - \bar {\bs u}_i \|_1 + \lambda \| s( {\bs u}_{i_t+1} - {\bs u}_{i_t}) \|_\infty \|{\bs u}_{i_t} - \bar {\bs u}_i \|_1 + \lambda C_i,\\
    &\le 3\lambda C_i.
\end{align}

So we have,
\begin{align}
    T_{3,i}
    &\le \frac{\beta n_i C_i^2}{2} + 3 \lamda C_i,\\
    &\le \beta/2 + 3 \lamda C_i,
\end{align}
where we used $C_i \le 1/\sqrt{n_i}$ by construction. From Lemma \ref{lem:t2-sc-d} we have,
\begin{align}
    T_{2,i}
    &\le \frac{-\lambda^2 \|\Delta \bs s_i\|_2^2}{2n_i \beta} + \lambda \|\Delta \bs s_i\|_2 C_i.
\end{align}

So,
\begin{align}
    T_{2,i} + T_{3,i}
    &\le \beta/2 -  \frac{\lambda^2 \|\Delta \bs s_i\|_2^2}{2n_i \beta} + 2\lambda (\|\Delta \bs s_i\|_2 \vee 3) C_i,\\
    &= \beta/2 - \left( \frac{\lamda \|\Delta \bs s_i\|_2}{\sqrt{2 n_i \beta}} - \frac{(\|\Delta \bs s_i\|_2 \vee 3) C_i \sqrt{2 n_i \beta}}{\|\Delta \bs s_i\|_2}\right)^2 +  2\left(\frac{\|\Delta \bs s_i\|_2 \vee 3}{\|\Delta \bs s_i\|_2}\right)^2  \beta n_i C_i^2,\\
    &\le \beta/2 + 2\left(\frac{\|\Delta \bs s_i\|_2 \vee 3}{\|\Delta \bs s_i\|_2}\right)^2  \beta n_i C_i^2,\\
    &\le 37\beta,
\end{align}-
where we used the fact that $\frac{\|\Delta \bs s_i\|_2 \vee 3}{\|\Delta \bs s_i\|_2} \le 6$ by the virtue of $\|\Delta \bs s_i\|_2 \ge \|\Delta \bs s_i\|_\infty \ge 1/2$. The splitting in Step 2 of Proposition \ref{prop:key-part} was done to ensure such a lower bound on $\|\Delta \bs s_i\|_\infty$. Combining Lemma \ref{lem:t1-sc-d} we can bound the total regret incurred within bin $i$ as:

\begin{align}
    T_{1,i} +  T_{2,i} + T_{3,i}
    &= O \left(\frac{G^2}{H} \log n  + \beta \right). \label{eqn:reg1}
\end{align}

Next we address bins that are derived from the elements of set $\mathcal Q$ in Step 3. We start from an alternate bound on $T_{2,i}$ as follows.

\begin{align}
    T_{2,i}
    &\le \frac{-\lambda^2 \|\Delta \bs s_i\|_2^2}{2n_i \beta} + \lambda \|\Delta \bs s_i\|_1 C_i. \label{eqn:alt-t2}
\end{align}

We also have,
\begin{align}
    T_{3,i}
    &\le \left(\sum_{k=1}^{d} \frac{\beta n_i C_i^2}{2d} \right) + \lambda \left( \langle s( {\bs u}_{i_s} - {\bs u}_{i_s-1}), {\bs u}_{i_s} - \bar {\bs u}_i \rangle - \langle s({\bs u}_{i_t + 1} - {\bs u}_{i_t}) , {\bs u}_{i_t} - \bar {\bs u}_i \rangle \right) \\ &\qquad +\lambda \sum_{j=i_s+1}^{i_t} |{\bs u}_j - {\bs u}_{j-1}|, \label{eqn:alt-t3}
\end{align}

We notice that Eq. \eqref{eqn:alt-t2} and Eq \eqref{eqn:alt-t3} decomposes per-coordinate basis. So for a coordinate $k \in [d]$, define,
\begin{align}
    S_{k,i}
    &:= \frac{-\lambda^2  (\Delta \bs s_i[k])^2}{2n_i \beta} + \lamda |\Delta \bs s_i[k]| C_i + \frac{\beta n_i C_i^2}{2d} +\lamda \sum_{j=i_s+1}^{i_t} |{\bs u}_j[k] - {\bs u}_{j-1}[k]|\\
    &\qquad+ \lamda \left(  s( {\bs u}_{i_s}[k] - {\bs u}_{i_s-1}[k]) ({\bs u}_{i_s}[k] - \bar {\bs u}_i[k]) -  s({\bs u}_{i_t + 1}[k] - {\bs u}_{i_t}[k]) ({\bs u}_{i_t}[k] - \bar {\bs u}_i[k])\right). \label{eqn:cord-regret}
\end{align}
We proceed to bound each term $S_{k,i}$.

After running Steps 3-5, let a bin $[\ubar t,\bar t] \in \mathcal Q$ be split into consecutive bins viz $\mathcal A = \{ [\ubar t,\ubar t_{-p} -1], [\ubar t_{-p}, \bar t_{-p}], \ldots [\ubar t_0, \bar t_0] \}$ and $\mathcal B = \{[\ubar t_1,\bar t_1],\ldots, [\ubar t_m,\bar t_m] \}$ and $\mathcal C = \{ [\ubar t_{m+1},\bar t_{m+1}],\ldots,[\bar t_q + 1,\bar t] \}$. The offline optimal sequence satisfies the following properties:
\begin{enumerate}
    \item $\bs u[k]$ is constant in $[\ubar t,\bar t_0]$.
    \item $\bs u_{\ubar t_1}[k] > \bs u_{\bar t_0}[k]$ and $\bs u_{\ubar t_{m+1}}[k] > \bs u_{\bar t_m}[k]$.
    \item $\bs u[k]$ is non-decreasing in $[\ubar t_1, \bar t_m]$.
    \item $\bs u[k]$ is constant in $[\ubar t_{m+1},\bar t]$.
\end{enumerate}

Note that by construction $|\mathcal A|+|\mathcal B|+|\mathcal C| = O(d)$. We remark that all the arguments for the case when $>$ is replaced by $<$ in (2) and non-decreasing is replaced by non-increasing in (3) are similar to the case considered above.

For notational consistency, let's annotate $[\ubar t,\ubar t_{-p} -1]$ by the number $-p-1$, $[\ubar t_{-p}, \bar t_{-p}]$ by $p$ and so on till $[\ubar t_q, \bar t_q]$ by $q$ and $[\bar t_q + 1,\bar t]$ by $q+1$.

First we focus on the partitions in $\mathcal B$. Let $n_{\ubar t1 \rightarrow \bar t_m} := \bar t_m - \ubar t_1 + 1$. Let $C_{\ubar t_1 \rightarrow \bar t_m}$ be the TV of the offline optimal in bin $[\ubar t_1, \bar t_m]$ which by construction is at-most $1/\sqrt{l_t}$, where $l_t := \bar t - \ubar t +1$. We have,
\begin{align}
    \sum_{j=1}^{m} S_{k,j}
    &\le \frac{\beta n_{\ubar t1 \rightarrow \bar t_m} C_{\ubar t_1 \rightarrow \bar t_m}^2}{2d} + \lamda C_{\ubar t_1 \rightarrow \bar t_m} + \lamda \left(s(\bs u_{\ubar t_1}[k] - \bs u_{\ubar t_1 - 1}[k]) \bs u_{\ubar t_1}[k]  - s(\bs u_{\bar t_m+1}[k] - \bs u_{\bar t_m}[k]) \bs u_{\bar t_m}[k]\right) \\
    &\qquad +\sum_{j=1}^{m} \frac{-\lambda^2  (\Delta \bs s_j[k])^2}{2n_j \beta} + \lamda |\Delta \bs s_j[k]| C_{\ubar t_1 \rightarrow \bar t_m} + \lamda \bar {\bs u}_j[k]  \Delta \bs s_j[k],\\
    &\le_{(a)} \frac{\beta l_{t} C_{t}^2}{2d} + \lamda C_{\ubar t_1 \rightarrow \bar t_m} + \lamda \left(s(\bs u_{\ubar t_1}[k] - \bs u_{\ubar t_1 - 1}[k]) \bs u_{\ubar t_1}[k]  - s(\bs u_{\bar t_m+1}[k] - \bs u_{\bar t_m}[k]) \bs u_{\bar t_m}[k]\right) \\
    &\qquad +\sum_{j=1}^{m} \frac{-\lambda^2  (\Delta \bs s_j[k])^2}{2n_j \beta} + \lamda |\Delta \bs s_j[k]| C_{t} + \lamda \bar {\bs u}_j[k]  \Delta \bs s_j[k],\\
    &\le_{(b)} \frac{\beta}{2d} +\sum_{j=1}^{m} \frac{-\lambda^2  (\Delta \bs s_j[k])^2}{2n_j \beta} + \lamda |\Delta \bs s_j[k]| C_{t} + \lamda \bar {\bs u}_j[k]  \Delta \bs s_j[k],    
\end{align}
where in line (a) we used the fact that $C_{\ubar t_1 \rightarrow \bar t_m} \le C_t$ since $[\ubar t_1,\bar t_m]$ is contained within $[\ubar t, \bar t]$. In line (b) we used $C_t \le 1/\sqrt{l_t}$ along with the fact that \\$\lamda \left(s(\bs u_{\ubar t_1}[k] - \bs u_{\ubar t_1 - 1}[k]) \bs u_{\ubar t_1}[k]  - s(\bs u_{\bar t_m+1}[k] - \bs u_{\bar t_m}[k]) \bs u_{\bar t_m}[k]\right) = -\lamda C_{\ubar t_1 \rightarrow \bar t_m}$ since \\
$s(\bs u_{\ubar t_1}[k] - \bs u_{\ubar t_1 - 1}[k]) = s(\bs u_{\bar t_m+1}[k] - \bs u_{\bar t_m}[k]) = 1$ and the sequence $\bs u[k]$ is non-decreasing in $[\ubar t_1, \bar t_m]$.

Observe that since $s(\bs u_{\ubar t_1}[k] - \bs u_{\ubar t_1 - 1}[k]) = s(\bs u_{\bar t_m+1}[k] - \bs u_{\bar t_m}[k]) = 1$, we can write\\ $\sum_{j=1}^{m} \Delta \bs s_j[k] = 0$. Define $\check{ \bs u}_{\mathcal B} := \frac{1}{m} \sum_{j=1}^{m} \bar {\bs u}_j$. We have,

\begin{align}
     \sum_{j=1}^{m} S_{k,j}
     &\le \frac{\beta}{2d} +\sum_{j=1}^{m} \frac{-\lambda^2  (\Delta \bs s_j[k])^2}{2n_j \beta} + \lamda |\Delta \bs s_j[k]| C_{t} + \lamda \left(\bar {\bs u}_j[k] - \check{ \bs u}_{\mathcal B}[k] \right)\Delta \bs s_j[k],\\
     &\le \frac{\beta}{2d} +\sum_{j=1}^{m} \frac{-\lambda^2  (\Delta \bs s_j[k])^2}{2n_j \beta} + 2 \lamda |\Delta \bs s_j[k]| C_{t},\\
     &= \frac{\beta}{2d} +\sum_{j=1}^{m} -\left(\frac{\lamda \Delta \bs s_j[k]}{\sqrt{2 n_j \beta}}  - C_t \sqrt{2 n_j \beta}\right)^2 + 2\beta n_j C_t^2,\\
     &\le \frac{\beta}{2d} + 2\beta,\\
     &\le 3\beta.
\end{align}

We remark that the key ingredient that made this possible is the fact that $s(\bs u_{\ubar t_1}[k] - \bs u_{\ubar t_1 - 1}[k]) = s(\bs u_{\bar t_m+1}[k] - \bs u_{\bar t_m}[k]) = 1 (\text{or } -1)$ for the non-decreasing (or non-increasing)  sequence $\bs u$ in $[\ubar t_1,\bar t_m]$. This is the reason behind the design of steps (i) and (ii) in Proposition \ref{prop:key-part}.

Next, we address bins present in $\mathcal A$ and $\mathcal C$. We provide the arguments for bounding $\sum_{j=-p-1}^{0} S_{k,j}$. Bounding the sum for bins in $\mathcal C$ can be done using similar arguments.

Observe that by the construction in Proposition \ref{prop:key-part}, the sequence $\bs u_t[k]$ for $t \in [i_s,\bar t_0]$ is a constant. So the last two terms in Eq. \eqref{eqn:cord-regret} is zero for any $S_{k,j}, j \in [-p-1,0]$. Now proceeding similar to above by completing the squares and dropping the negative terms, we get

\begin{align}
    \sum_{j=-p-1}^{0} S_{k,j}
    &\le \frac{\beta}{2d} +\sum_{j=-p-1}^{0} -\left(\frac{\lamda \Delta \bs s_j[k]}{\sqrt{2 n_j \beta}}  - C_t \sqrt{n_j \beta/2}\right)^2 + \beta n_j C_t^2/2,\\
    &\le \beta.
\end{align}

Combining Lemma \ref{lem:t1-sc-d} and noting that  $|\mathcal A|+|\mathcal B|+|\mathcal C| = O(d)$ we can bound the total regret incurred within bin $[\ubar t, \bar t]$ (denoted by $R[\ubar t, \bar t]$) as

\begin{align}
    R[\ubar t, \bar t]
    &\le O \left(\frac{d G^2}{H} \log n \right) + \sum_{k=1}^{d} \sum_{j=-p-1}^{q+1} S_{k,j},\\
    &\le O \left(\frac{d G^2}{H} \log n + d \beta \right) \label{eqn:reg2}.
\end{align}

As noted in the proof of Lemma \ref{lem:num-bins}, there are only $O(n^{1/3}C_n^{2/3})$ bins in $\cP$ at the end of Step 2 in Proposition \ref{prop:key-part}. Hence adding the bounds in Eq. \eqref{eqn:reg1} and \eqref{eqn:reg2} across those bins yields the Theorem.

\end{proof}
\end{comment}

